Contract Composition for Dynamical Control Systems: Definition and Verification using Linear Programming

Designing large-scale control systems to satisfy complex specifications is hard in practice, as most formal methods are limited to systems of modest size. Contract theory has been proposed as a modular alternative to formal methods in control, in which specifications are defined by assumptions on the input to a component and guarantees on its output. However, current contract-based methods for control systems either prescribe guarantees on the state of the system, going against the spirit of contract theory, or can only support rudimentary compositions. In this paper, we present a contract-based modular framework for discrete-time dynamical control systems. We extend the definition of contracts by allowing the assumption on the input at a time $k$ to depend on outputs up to time $k-1$, which is essential when considering the feedback connection of an unregulated dynamical system and a controller. We also define contract composition for arbitrary interconnection topologies, under the pretence of well-posedness, and prove that this notion supports modular design, analysis and verification. This is done using graph theory methods, and specifically using the notions of topological ordering and backward-reachable nodes. Lastly, we use $k$-induction to present an algorithm for verifying vertical contracts, which are claims of the form "the conjugation of given component-level contracts is a stronger specification than a given contract on the integrated system". These algorithms are based on linear programming, and scale linearly with the number of components in the interconnected network. A numerical example is provided to demonstrate the scalability of the presented approach, as well as the modularity achieved by using it.

==> Aux tex files/Old_2SysCascade.tex <==
\section{Two Systems in Cascade} \label{sec.Cascade}



The proof of the theorem can be found in Appendix \ref{appendix.Vert}. The theorem allows one to verify that a given composition of cascaded contracts refines a contract on the composite system by verifying three implications, each of them can be cast as a linear program:
\begin{subequations} \label{eq.LP_TwoSystemCascade}
\begin{align}
    \varrho_1 = \max ~&~ \max_{\ell = m - m_1,\ldots,m}\alpha_1(d_1(\ell-m_1:\ell))\\ \nonumber
    {\rm s.t.}~&~ \alpha_{\rm tot}(d_1(\ell - m_{\rm tot}:\ell)) \le 0,~~~\forall \ell = m_{\rm tot},\ldots,m\\\nonumber
    ~&~ d_1(0:m) \in (\R^{n_{d_1}})^{m+1}
\end{align}
\begin{align}
    \varrho_2 = \max ~&~  \max_{\ell = m - m_2,\ldots, m}\alpha_2(y_1(\ell-m_2:\ell))\\\nonumber
    {\rm s.t.}~&~  \alpha_{\rm tot}(d_1(\ell - m_{\rm tot}:\ell)) \le 0,~~~\forall \ell = m_{\rm tot},\ldots,m\\\nonumber
    ~&~\gamma_1\left(\begin{smallmatrix}d_1(\ell-m_1:\ell) \\ y_1(\ell - m_1:\ell)\end{smallmatrix}\right) \le 0,~~~~~~~~~~\forall \ell = m_1,\ldots,m,\\\nonumber
    ~&~ d_1(0:m) \in (\R^{n_{d_1}})^{m+1},y_1(0:m) \in (\R^{n_{y_1}})^{m+1}
\end{align}
\begin{align}
    \varrho_\OO = \max ~&~ \max_{\ell = m_{\rm tot},\ldots,m}\gamma_{\rm tot}\left(\begin{smallmatrix}d_1(\ell-m_{\rm tot}:\ell) \\ \nonumber y_2(\ell-m_{\rm tot}:\ell)\end{smallmatrix}\right)\\
    {\rm s.t.}~&~ \alpha_1(d_1(\ell - m_1:\ell)) \le 0,~~~ \forall \ell = m_{\rm tot},\ldots,m\\ \nonumber
    ~&~\gamma_1\left(\begin{smallmatrix}d_1(\ell - m_1:\ell) \\ y_1(\ell - m_1:\ell)\end{smallmatrix}\right) \le 0,~~~~~~\forall \ell = m_1,\ldots,m\\ \nonumber
    ~&~\gamma_2\left(\begin{smallmatrix}y_1(\ell - m_2:\ell) \\ y_2(\ell - m_2:\ell)\end{smallmatrix}\right) \le 0,~~~~~~\forall \ell = m_2,\ldots,m\\ \nonumber
    ~&~ d_1(0:m) \in (\R^{n_{d_1}})^{m+1},y_1(0:m) \in (\R^{n_{y_1}})^{m+1}\\ \nonumber
    ~&~ y_2(0:m) \in (\R^{n_{y_2}})^{m+1}
\end{align}
\end{subequations}
These suggest the following algorithm for determining whether $\C_1 \otimes \C_2 \preccurlyeq \C_{\rm tot}$:

\begin{algorithm} [h]
\caption{Verifying Vertical Contracts - Two-System Cascade Composition}
\label{alg.VerifyTwoSysCascade}
{\bf Input:} Three LTI contracts $\C_1,\C_2,\C_{\rm tot}$ given by \eqref{eq.ThreeContractsCascade}, where $\C_1,\C_2$ are in feedback as in Fig. \ref{fig.CascadeTwoSystems} and $\C_{\rm tot}$ is a contract on the composite system\\
{\bf Output:} A boolean variable, determining whether $\C_1 \otimes \C_2 \preccurlyeq \C_{\rm tot}$.
\begin{algorithmic}[1]
\State Compute $\varrho_1,\varrho_2,\varrho_\OO$ by solving the linear programs in \eqref{eq.LP_TwoSystemCascade}.
\If{$\varrho_1,\varrho_2,\varrho_\OO$ are non-negative}
\State {\bf Return} true.
\Else
\State {\bf Return} false.
\EndIf
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg.VerifyTwoSysCascade} presents a computationally viable verification method for cascaded vertical contracts, and can be applied using off-the shelf optimization software, e.g. Yalmip \cite{Lofberg2004}. Its correctness is shown in the following theorem:

\begin{thm} \label{thm.Opt}
Suppose that the assumptions of Theorem \ref{thm.VertCascadeTwo} hold. Then Algorithm \ref{alg.VerifyTwoSysCascade} is always correct, i.e. the cascaded vertical contract $\C_1 \otimes \C_2 \preccurlyeq \C_{\rm tot}$ holds if and only if the algorithm returns ``true".
\end{thm}

\begin{proof}
Implication i) in Theorem \ref{thm.VertCascadeTwo} holds if and only if $ \alpha_1(d_1(0:m_1)) \le 0$ holds whenever $\alpha_{\rm tot}(d_1(\ell - m_{\rm tot}:\ell)) \le 0$ holds for all $\ell = m_{\rm tot},\ldots,m$. This implication is true if and only if $\varrho_1 \le 0$. Similarly, implication ii) holds if and only if $\varrho_2 \le 0$, and implication iii) in holds if and only if $\varrho_{\OO}\le 0$.
\end{proof}

==> Aux tex files/Old_2SysFeedback.tex <==
\section{Two Systems in Feedback} \label{sec.TwoFeedback}

\begin{thm} \label{thm.InductionTruncation}
If any of the implications (I.1), (I.2) or (II) holds for $n=m-1$, then they hold for any $n\in \N, n\ge m-1$.
\end{thm}

\begin{proof}
We focus on the implication (I.1) for conciseness, as the proof of the fact for all three collections of implications is nearly identical. The proof uses induction on the time $n$, where the induction base holds by assumption.

We assume that the implication (I.1) holds for some value of $n$, and prove it for $n+1$. Thus, we take arbitrary $d(0:n+2),y(0:n+2),u(0:n+2)$ satisfying 
\begin{align*}
    \begin{cases}
        \alpha_{\rm tot}(d(k-m_{\rm tot}:k)) \le 0& ,\forall k = m_{\rm tot},\ldots,{n+2}\\
        \gamma_1\left(\begin{smallmatrix} d(k-m_1:k) \\ u(k-m_1:k-1) \\ y(k-m_1:k) \end{smallmatrix}\right) \le 0&,\forall k = m_1,\ldots,n+1\\
        \gamma_2\left(\begin{smallmatrix} y(k-m_1:k) \\ u(k-m_1:k)\end{smallmatrix}\right) \le 0&, \forall k = m_2,\ldots,n+2,
    \end{cases}
\end{align*}
and we want to show that $\alpha_1\left(\begin{smallmatrix} d(\ell-m_1:\ell) \\ u(\ell-m_1:\ell-1) \end{smallmatrix}\right)\le 0$ holds for $\ell = m_1,\ldots,n+2$. The inequality immediately follows for $\ell = m_1,\ldots,n+1$ from the induction hypothesis, so we focus on proving that $\alpha_1\left(\begin{smallmatrix} d(n+2-m_1:n+2) \\ u(n+2-m_1:n+1) \end{smallmatrix}\right)\le 0$.

We consider the shifted (and truncated) signals $\hat{d},\hat{y}$ and $\hat{u}$ as $\hat{d}(0:n+1) = d(1:n+2), \hat{y}(0:n+1) = y(1:n+2)$ and $\hat{u}(0:n+1)$. By definition, we note that:
\begin{align*}
    \begin{cases}
        \alpha_{\rm tot}(\hat d(k-m_{\rm tot}:k)) \le 0& ,\forall k = m_{\rm tot},\ldots,{n+1}\\
        \gamma_1\left(\begin{smallmatrix} \hat d(k-m_1:k) \\ \hat u(k-m_1:k-1) \\ \hat y(k-m_1:k) \end{smallmatrix}\right) \le 0&,\forall k = m_1,\ldots,n\\
        \gamma_2\left(\begin{smallmatrix} \hat y(k-m_1:k) \\ \hat u(k-m_1:k)\end{smallmatrix}\right) \le 0&, \forall k = m_2,\ldots,n+1.
    \end{cases}
\end{align*}
Thus, we conclude that
$\alpha_1\left(\begin{smallmatrix} d(n+2-m_1:n+2) \\ u(n+2-m_1:n+1) \end{smallmatrix}\right) = \alpha_1\left(\begin{smallmatrix} \hat d(n+1-m_1:n+1) \\ \hat u(n+1-m_1:n) \end{smallmatrix}\right)\le 0$ using the induction hypothesis.
\end{proof}

Combining Theorem \ref{thm.VerticalFeedbackContracts} and Theorem \ref{thm.InductionTruncation}, we conclude that $\C_1\otimes \C_2 \preccurlyeq \C_{\rm tot}$ is equivalent to three implications between linear inequalities, namely (I.1), (I.2) and (II) for $n=m-1$. Similarly to the previous sections, these implications can be recasted as linear programs:
\begin{subequations} \label{eq.LP_TwoSystemFeedback}
\begin{align}
    \varrho_1 = \max ~&~ \max_{\ell = m_1,\ldots,m}\alpha_1\left(\begin{smallmatrix} d(\ell-m_1:\ell) \\ u(\ell-m_1:\ell-1) \end{smallmatrix}\right)\\\nonumber
    {\rm s.t.}~&~ \alpha_{\rm tot}(d(\ell-m_{\rm tot}:\ell)) \le 0~~ ,\forall \ell = m_{\rm tot},\ldots,m\\\nonumber
    ~&~\gamma_1\left(\begin{smallmatrix} d(\ell-m_1:\ell) \\ u(\ell-m_1:\ell-1) \\ y(\ell-m_1:\ell) \end{smallmatrix}\right) \le 0\hspace{.58cm},\forall \ell = m_1,\ldots,m-1\\\nonumber
    ~&~\gamma_2\left(\begin{smallmatrix} y(\ell-m_1:\ell) \\ u(\ell-m_1:\ell)\end{smallmatrix}\right) \le 0 \hspace{1.03cm}, \forall \ell = m_2,\ldots,m-1\\\nonumber
    ~&~ d(0:m)\in (\R^{n_d})^{m+1},&&\\\nonumber
    ~&~ y(0:m)\in (\R^{n_d})^{m+1},&&\\\nonumber
    ~&~ u(0:m)\in (\R^{n_d})^{m+1},&&
\end{align}
\begin{align}
    \varrho_2 = \max ~&~  \max_{\ell = m_2,\ldots,m}\alpha_2(y(\ell-m_2:\ell))\\\nonumber
    {\rm s.t.}~&~ \alpha_{\rm tot}(d(\ell-m_{\rm tot}:\ell)) \le 0~~,\forall \ell = m_{\rm tot},\ldots,m\\\nonumber
    ~&~\gamma_1\left(\begin{smallmatrix} d(\ell-m_1:\ell) \\ u(\ell-m_1:\ell-1) \\ y(\ell-m_1:\ell) \end{smallmatrix}\right) \le 0\hspace{.58cm},\forall \ell = m_1,\ldots,m\\\nonumber
    ~&~\gamma_2\left(\begin{smallmatrix} y(\ell-m_1:\ell) \\ u(\ell-m_1:\ell)\end{smallmatrix}\right) \le 0\hspace{1.03cm}, \forall \ell = m_2,\ldots,m-1\\\nonumber
    ~&~ d(0:m)\in (\R^{n_d})^{m+1},&&\\\nonumber
    ~&~ y(0:m)\in (\R^{n_d})^{m+1},&&\\\nonumber
    ~&~ u(0:m)\in (\R^{n_d})^{m+1},&&
\end{align}
\begin{align}
    \varrho_\OO = \max ~&~ \max_{\ell = m_{\rm tot},\ldots,m}\gamma_{\rm tot}\left(\begin{smallmatrix} d(\ell-m_{\rm tot}:\ell) \\ y(\ell-m_{\rm tot}:\ell) \end{smallmatrix}\right)\\\nonumber
    {\rm s.t.}~&~ \alpha_{\rm tot}(d(\ell-m_{\rm tot}:\ell)) \le 0~~~~ ,\forall \ell = m_{\rm tot},\ldots,m\\\nonumber
    ~&~\gamma_1\left(\begin{smallmatrix} d(\ell-m_1:\ell) \\ u(\ell-m_1:\ell-1) \\ y(\ell-m_1:\ell) \end{smallmatrix}\right) \le 0\hspace{.83cm},\forall \ell = m_1,\ldots,m\\\nonumber
    ~&~\gamma_2\left(\begin{smallmatrix} y(\ell-m_1:\ell) \\ u(\ell-m_1:\ell)\end{smallmatrix}\right) \le 0\hspace{1.28cm}, \forall \ell = m_2,\ldots,m\\\nonumber
    ~&~ d(0:m)\in (\R^{n_d})^{m+1},&&\\\nonumber
    ~&~ y(0:m)\in (\R^{n_d})^{m+1},&&\\\nonumber
    ~&~ u(0:m)\in (\R^{n_d})^{m+1}.&&
\end{align}
\end{subequations}
These suggest the following algorithm for determining whether $\C_1 \otimes \C_2 \preccurlyeq \C_{\rm tot}$:

\begin{algorithm} [h]
\caption{Verifying Vertical Contracts - Two-System Feedback Composition}
\label{alg.VerifyTwoSysFeedback}
{\bf Input:} Three LTI contracts $\C_1,\C_2,\C_{\rm tot}$ given by \eqref{eq.ThreeRDSCContracts}, where $\C_1,\C_2$ are in feedback as in Fig. \ref{fig.FeedbackTwoSystems} and $\C_{\rm tot}$ is a contract on the composite system\\
{\bf Output:} A boolean variable, determining whether $\C_1 \otimes \C_2 \preccurlyeq \C$.
\begin{algorithmic}[1]
\State Compute $\varrho_1,\varrho_2,\varrho_\OO$ by solving the linear programs in \eqref{eq.LP_TwoSystemFeedback}.
\If{$\varrho_1,\varrho_2,\varrho_\OO$ are non-negative}
\State {\bf Return} true.
\Else
\State {\bf Return} false.
\EndIf
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg.VerifyTwoSysFeedback} suggests a simple LP-based technique of checking whether a feedback vertical contract $\C_1 \otimes \C_2 \preccurlyeq \C_{\rm tot}$ holds by solving three linear programs, which can be done using widely available optimization software, e.g. Yalmip \cite{Lofberg2004}. The correctness of the algorithm can be proved:

\begin{thm}
Under the assumptions of Theorem \ref{thm.VerticalFeedbackContracts}, Algorithm \ref{alg.VerifyTwoSysFeedback} is always correct, i.e. $\C_1\otimes \C_2 \preccurlyeq \C_{\rm tot}$ holds if and only if the algorithm returns ``true".
\end{thm}
\begin{proof}
Similarly to Theorem \ref{thm.Opt}.
\end{proof}

